Throughput-Improving Control of Highways Facing Stochastic Perturbations

In this paper, we study the problem of traffic management in highways facing stochastic perturbations. To model the macroscopic traffic flow under perturbations, we use cell-transmission model with Markovian capacities. The decision variables are: (i) the admissible flow through each on-ramp, and (ii) whether individual on-ramps are metered to prioritize the mainline traffic or not. The objective is to maximize the throughput while ensuring that on-ramp queues remain bounded on average. We develop a computational approach to solving this stability-constrained, throughput-maximization problem. We establish a mixed-integer linear program for throughput maximization and construct an algorithm that gives the optimal solution in particular settings. We illustrate the performance benefits of the proposed approach through a computational study on a segment of Interstate 210 in California, USA.

==> Texts/05_Abstract.tex <==
\begin{abstract}
In this article, we study the problem of controlling a highway segment facing stochastic perturbations, such as recurrent incidents and moving bottlenecks. To model traffic flow under perturbations, we use the cell-transmission model with Markovian capacities.  The control inputs are: (i) the inflows that are sent to various on-ramps to the highway (for managing traffic demand), and (ii) the priority levels assigned to the on-ramp traffic relative to the mainline traffic (for allocating highway capacity). The objective is to maximize the throughput while ensuring that on-ramp queues remain bounded in the long-run. We develop a computational approach to solving this stability-constrained, throughput-maximization problem. Firstly, we use the classical drift condition in stability analysis of Markov processes to derive a sufficient condition for boundedness of on-ramp queues. Secondly, we show that our control design problem can be formulated as a mixed integer program with linear or bilinear constraints, depending on the complexity of Lyapunov function involved in the stability condition. Finally, for specific types of capacity perturbations, we derive intuitive criteria for managing demand and/or selecting priority levels. These criteria suggest that inflows and priority levels should be determined simultaneously such that traffic queues are placed at locations that discharge queues fast. We illustrate the performance benefits of these criteria through a computational study of a segment on Interstate 210 in California, USA. 
\end{abstract}

\textbf{Index terms}:
Traffic control, Piecewise-deterministic Markov processes, Stability analysis.

==> Texts/Acknowledge.tex <==
\section*{Acknowledgement}
This work was supported by NYU Tandon School of Engineering, C2SMART University Transportation Center, US NSF CAREER Award CNS-1453126, and Singapore NRF Future Urban Mobility.
Ms. Sijia Liu at NYU Center for Data Science contributed to the simulation.
We also appreciate the discussion with Prof. Pravin Varaiya and Dr. Gabriel Gomes and the valuable inputs from the anonymous reviewers and the associate editor.

==> Texts/Appx.tex <==
%\begin{appendices}
%\footnotesize
\section*{Appendices}
\emph{A1 $\ $ Invariant set}
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Invariant set}
\label{sub_invariant}

%Following \cite{benaim15}, a set $\mathcal M\subseteq\mathcal Q\times\mathcal N$ is a {globally attracting and positively invariant set} for the continuous state $x=(q,n)$ if
%\begin{subequations}
%\begin{align}
%&\forall(I(0),X(0))\in \I\times (\Q\times\N),\ 
%\forall\epsilon>0,\ \exists T\ge0,\nonumber\\
%&\qquad \forall t\ge T,\ %\nonumber\\
%%&\quad
%\min_{x\in{\mathcal M}}\|(X(t))-x\|_2\le\epsilon,
%\label{Eq_Attracting}\\
%& \forall(I(0),X(0))\in \I\times{\mathcal M},  \forall t\ge0,\ 
%(X(t))\in{\mathcal M}.\label{Eq_Invariant0}
%\end{align}
%\label{Eq_Invariant}%
%\end{subequations}
%Intuitively, ${\mathcal M}$ is a set of states such that, for all initial conditions $(i,q,n)\in\mathcal I\times\mathcal Q\times\mathcal N$, the process $(I(t),Q(t),N(t))$ eventually enters and does not leave $\mathcal M$.
%For convenience, we henceforth refer to any set satisfying \eqref{Eq_Attracting}--\eqref{Eq_Invariant0} simply as an \emph{invariant set}.

For a given control input $u\in[0,d]\times\{0,1\}^K$, we explicitly construct an invariant set of the continuous state $x=(q,n)$ as follows:
$
{\mathcal M}(u):=
\bigcup_{{q}\in\prod_{k=1}^K[\bunderline q_k(u),\bar q_k(u)]}\Big(\{q\}\times\prod_{k=1}^K[\nbot_k({q},u),\ntop_k(u)]\Big),
$
where
{\scriptsize
\begin{align*}
%qbot
&\bunderline q_k(u):=\left\{\begin{array}{ll}
\infty & \mbox{if } v_k> {\mathsf R}_k\\
0 & \mbox{o.w.}
\end{array}\right.
\quad k=1,\ldots,K,\\
%rhobot
&\nbot_1({q},u):=\left\{\begin{array}{ll}
v_1/\alpha_1 & \mbox{if } {q}_1=0\\
\mathsf R_1/\alpha_1,& \mbox{o.w.}
\end{array}\right.\\
&\color{MidnightBlue}\nbot_k({q},u):=\left\{\begin{array}{ll}
\min\{\rho_{k-1}\nbot_{k-1}(q,u)+\frac{v_k}{\alpha_k},\frac{{\mathsf F}_k}{\alpha_k}\}
& \mbox{if } {q}_k=0\\
\min\{\rho_{k-1}\nbot_{k-1}(q,u)+\frac{{\mathsf R}_k}{\alpha_k},\frac{{\mathsf F}_k}{\alpha_k}\} &
\mbox{o.w.}
\end{array}\right.\\
&\color{MidnightBlue}\hspace{4.5cm} k=2,\ldots,K,\mbox{/2.12/}\\
%rhotop
&\ntop_K(u):={n}^\max_K-\min_iF_K(i)/\beta_K,\\
&\ntop_k(u):=\min\Bigg\{\frac{{\mathsf F}_k}{\alpha_k},{n}^\max_k-\frac{\min_iF_k(i)}{\beta_k},{n}^\max_k\\
&\hspace{2.5cm}-\frac{{\beta_{k+1}(n^{\max}_{k+1}-\ntop_{k+1}(u))-v_{k+1}w_{k+1}}}{\rho_k\beta_k}\Bigg\}
\\
&\hspace{1in}
k=K-1,K-2,\ldots,1, \\
%qtop
&\bar q_k(u):=\left\{\begin{array}{ll}
0 & \mbox{if } v_k\le{\mathsf R}_k\mbox{ and }v_k\le\beta_k(n^\max_k-\bar n_k(u))\\
&\;-(1-w_k)\rho_{k-1}\min\{\alpha_{k-1} \bar n_{k-1}(u),{\mathsf F}_k\}\\
\infty & \mbox{o.w.}
\end{array}\right.\\
&\hspace{5cm} k=1,\ldots,K.
\end{align*}}
{\color{MidnightBlue}/2.7/The upper bounds for $n_k$ are computed assuming maximal downstream congestion, and the lower bounds are computed assuming minimal upstream flow.
/2.13/For ease of presentation, we assume that $d$ is such that $\bar q_k=0$ if $w_k=1$; that is, if an on-ramp is prioritized over the mainline, then no queue will be formed there.
}
Furthermore, we can partition ${\mathcal M}$ into two subsets:
\begin{subequations}
\begin{align}
&{\mathcal M}_0(u):=\{(q,n)\in\mathcal M(u):q=0\},\label{eq_M0}\\
&{\mathcal M}_1(u):=\{(q,n)\in\mathcal M(u):q\neq0\},\label{eq_M1}
\end{align}
\end{subequations}
{\color{MidnightBlue}/2.12/where $q=0$ means that $q$ is the vector of zeros.}

%Note that the invariant set $\mathcal M(u)$ may or may not be bounded: $\mathcal M(u)$ is bounded if and only if $\bar q_k=0$ for all $k$.
%A bounded invariant set immediately imply stability of the SS-CTM. 
%%Thus, we only need to focus on the case where $\mathcal M(u)$ is unbounded, i.e. $\bar q_k=\infty$ for some $k$; see \eqref{eq_qtop}.
%If $\mathcal M(u)$ is unbounded and only contains states with infinite norms, i.e. if $|q|=\infty$ for every $(q,n)\in\mathcal M(u)$, then we can immediately conclude instability of the SS-CTM. This case arises if and only if $\mathcal M_0(u)=\emptyset$.
%If $\mathcal M(u)$ is unbounded but contains states with finite norms, i.e. if both $\mathcal M_0(u)$ and $\mathcal M_1(u)$ are non-empty, then more work is needed for stability analysis; see the next subsection.
%The above conclusions are summarized by the result below:

%\begin{prp}[Invariant set]
%\label{prp_inv}
%For a given control input $u\in[0,d]\times\{0,1\}^K$, the set $\mathcal M(u)$ as defined in \eqref{eq_S} is globally attracting and positively invariant. Furthermore, the SS-CTM is 
% stable if $\mathcal M_1(u)=\emptyset$,
%and is unstable if $\mathcal M_0(u)=\emptyset$.
%\end{prp}

\emph{A2 $\ $ Mixed-integer linear reformulation of \eqref{eq_P1}}
{\scriptsize
\begin{subequations}
\begin{align}
\max&\ J=\sum_{k=1}^K{v}_k\tag{P2}\\
% drift
s.t.&\ \forall i\in\mathcal I,\ \forall{y}\in\{0,1\}^K\backslash\{0\}^K,\ \forall{z}\in\{0,1\}^K,\nonumber\\
&\;{a}_{h,1}{v}_1+\sum_{k=2}^{K}{a}_{h,k-1}{v}_k-\sum_{k=1}^{K-1}({a}_{h,k}-{a}_{h,k+1})
(\rho_k\tilde f_{k,y,z}^{(i)}\nonumber\\
&\qquad+\tilde r_{k+1,y,z}^{(i)})-{a}_{h,K}\tilde f_{k,y,z}^{(i)}
+\sum_{j\in\mathcal I}\nu_{ij}(b^{(j)}_h\nonumber\\
&\qquad-b^{(i)}_h)
\le-1+\sum_{k=1}^KM_1{y}_k{w}_k
\quad h=1,\ldots,K,\label{eq_drift2}
\\
%&{b}_i\ge0,\\
%r
&\; \tilde r_{k,y,z}^{(i)}\le {v}_k\quad\mbox{if }y_k=0,\
k=1,\ldots,K,\\
&\;\tilde r_{k,y,z}^{(i)}\le {\mathsf R}_k\quad
k=1,\ldots,K,\\
%f
&\;\tilde f_{k,y,z}^{(i)}\le
\rho_{h}^k\left(\min_iF_h(i)\right)+\sum_{\ell=h+1}^{k-1}\rho_{\ell}^k{{v}_\ell}+\tilde r_{k,y,z}^{(i)}\nonumber\\
&\qquad\mbox{if }z_k=0,\
h=1,\ldots, k-1,\
 k=1,\ldots,K,\\
 %
&\;\tilde f_{k,y,z}^{(i)}\le
\sum_{\ell=1}^{k-1}\rho_{\ell}^k{{v}_\ell}+\tilde r_{k,y,z}^{(i)}\ 
z_k=0,\
 k=1,\ldots,K,\\
% capacity
&\;\tilde f_{k,y,z}^{(i)}\le F_k(i) \quad
k=1,\ldots,K,\\
% if k+1 congested
&\;\tilde f_{k,y,z}^{(i)}\le
\frac{\tilde f_{k+1,y,z}^{(i)}-\tilde r_{k+1,y,z}^{(i)}}{\rho_k}\quad
\mbox{if }z_{k+1}=1,\nonumber\\
&\qquad k=1,\ldots,K-1,\\
%w
&\; {v}_k
\le \tilde f_{k,y,z}^{(i)}-\rho_{k-1}\tilde f_{k-1,y,z}^{(i)}+M_2w_k
+M_2(1-{\xi}_k)
\nonumber\\
&\qquad k=2,\ldots,K,
\\
&\; {v}_k
\le \tilde f_{k,y,z}^{(i)}+M_2(1-w_k)+M_2(1-{\xi}_k)\
 k=2,\ldots,K,
\\
% integers
&a_{kh}\ge{a}_{k+1,h}\quad
k=1,\ldots,K-1,
{a}_{Kh}\ge1\nonumber\\
&\quad h=1,\ldots,K,\
 v\in[0,d],\;w\in\{0,1\}^K,\;{\xi}\in\{0,1\}^K.
 \label{eq_uvw}
%
\end{align}
\end{subequations}}

==> Texts/Bio.tex <==
{\scriptsize
\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin2.jpg}}
\noindent \textbf{Li Jin} is an Assistant Professor in the Department of Civil and Urban Engineering at the New York University Tandon School of Engineering.
He received his B.Eng. in Mechanical Egineering from Shanghai Jiao Tong University in 2011, M.S. in Mechanical Egineering from Purdue University in 2012,  and Ph.D. in Transportation from the Massachusetts Institute of Technology in 2018.
%His research focuses on developing resilient control algorithms for cyber-physical systems with guarantees of efficiency in nominal settings, robustness against random perturbations, and survivability under strategic disruptions.
%The theoretical foundation of his work include stochastic process and control theory. 
%Specific applications of his work include connected and autonomous vehicles, automatic traffic control, air transportation, and gas network.
%He is a recipient of the Ho-Ching and Hang-Ching Fund Award and Schoettler Scholarship Fund.
}
%\vspace{4\baselineskip}

\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Kurzhanskiy.jpg}}
\noindent \textbf{Alexander A. Kurzhanskiy} is Assistant Research Engineer at University of California, Berkeley. He received his M.S. in Applied Mathematics from Lomonosov Moscow State University and his Ph.D. in Electrical Engineering \& Computer Science from Berkeley. From 1998 to 2003 he worked for several Silicon Valley companies.
%His research interests include dynamical systems estimation and control, application of the set-valued calculus to
%reachability analysis and estimation, robust convex optimization, transportation systems.
}
%\vspace{4\baselineskip}

\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Amin.jpg}}
\noindent \textbf{Saurabh Amin} is Robert an Associate Professor in the Department of Civil and Environmental Engineering and the and Institute of Data, Systems, and Society at the Massachusetts Institute of Technology. He received his Ph.D. from the University of California, Berkeley in 2011. 
His research focuses on the design of network inspection and control algorithms for infrastructure systems resilience. 
%He studies the effects of security attacks and natural events on the survivability of cyber-physical systems, and designs mechanisms to reduce network risks. 
%He is a recipient of NSF CAREER and Google Faculty Research awards.
}
}

==> Texts/Margin.tex <==
\section{Optimal control scheme: margin criterion}
\label{sec_optimal}

Although analytical solutions to the max-throughput problems may not be easy to obtain, we are able to characterize the optimal solutions under particular assumptions.
In this section, we study how capacity and demand jointly impact the structure of optimal ramp metering plans.
The main result of this section is that one can obtain a throughput-maximizing control scheme by applying the \emph{margin criterion}: the optimal priority at an on-ramp depends on the comparison between the capacity-demand margins of the on-ramp and of the mainline.

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stationary hotspot}
Based on Theorem~\ref{thm_stable1}, we now study how demand and capacity jointly determines the structure of an optimal traffic control scheme.
For each $(u,v)\in[0,d]\times\{0,1\}^K$, define
\begin{subequations}uti
\begin{align}
&\tilde F_1=F,\label{eq_Fhat1}\\
&\tilde F_k=\min\{F,v_k(u_k+\rho_{k-1}\tilde F_{k-1})+(1-v_k)(u+\sum_{h=1}^k\rho_h^ku_h)\},
\quad k=2,\ldots,K.\label{eq_Fhatk}
\end{align}
\end{subequations}
The interpretation of $\tilde F_k$ is as follows: if there exists congestion in an upstream cell, or if there exists a queue in an upstream buffer, then $\tilde F_k$ is the minimum rate at which traffic is discharged from cell $k$. $\tilde F_k$ can be viewed as a generalized notion of capacity: if cell $k$ is downstream to a bottleneck (either a mainline cell or an on-ramp buffer), then the discharged flow out of cell $k$ may depend on that bottleneck's capacity, rather than cell $k$'s capacity.
With $\tilde F_k$ defined as above, we have the following result:

\begin{prp}[Margin criterion, stationary]
\label{prp_ystar1}
For the throughput-maximizing problem \eqref{eq_thpmax1}, there exists an optimal scheme $(u^*,v^*)$ such that
\begin{align}
v_k^*=\left\{\begin{array}{ll}
0, & \rho_{k-1}(\tilde F_{k-1}-\sum_{h=1}^{k-1}\rho_h^{k-1}u_h^*)\le R-u_k^*,\\
1, & \mbox{o.w.}
\end{array}\right.
\quad k=2,\ldots,K,
\end{align}
where $\tilde F_k$ are given by \eqref{eq_Fhat1}--\eqref{eq_Fhatk}.
\end{prp}

Proposition~\ref{prp_ystar1} gives a criterion for whether to meter an on-ramp or not. Specifically, if an on-ramp has a capacity-demand margin $(R-u_k^*)$ that is larger than the capacity-demand margin ($F-\sum_{\ell=1}^{h}\rho_\ell^hu_\ell^*$) of some section $h$ on the mainline, then the on-ramp is supposed to be metered.
As an intuitive interpretation, if an on-ramp has a larger margin than the mainline, then the mainline is the ``bottleneck'' that imposes a stronger restriction on the throughput; in other words, the on-ramp can discharge traffic queue faster than the mainline does. Consequently, prioritizing the traffic from the bottleneck improves throughput.

{\bf Proof of Proposition~\ref{prp_ystar1}.}
Consider a given $u\in[0,d]$ a given $v\in\{0,1\}^K$.
To obtain the conclusion, we only need to show the following: If $(u,v)$ satisfies \eqref{eq_stable1a}--\eqref{eq_stable1z}, then,
\begin{enumerate}[(i)]
\item  if $v_k=1$ for some $2\le k\le K$, and if
    \begin{align}
    \rho_{k-1}(\tilde F_{k-1}-\sum_{h=1}^{k-1}\rho_h^{k-1}u_h)\le R-u_k,
    \label{eq_minF-x<}
    \end{align}
    then, for $v'=[v_1,\ldots,v_{k-1},0,v_{k+1},\ldots,v_K]^T$, $(u,v')$ also satisfies \eqref{eq_stable1a}--\eqref{eq_stable1z};
\item if $v_k=0$ for some $2\le k\le K$, and if
    \begin{align}
    \rho_{k-1}(\tilde F_{k-1}-\sum_{h=1}^{k-1}\rho_h^{k-1}u_h)\ge R-u_k,
    \label{eq_minF-x>}
    \end{align}
    then, for $v'=[v_1,\ldots,v_{k-1},1,v_{k+1},\ldots,v_K]^T$, $(u,v')$ also satisfies \eqref{eq_stable1a}--\eqref{eq_stable1z}.
\end{enumerate}

Here we only present the proof of part (i); part (ii) can be analogously proved.

Changing $v_k$ from 1 to 0 leads to the following changes. First, for \eqref{eq_stable1b}, the following constraint is added:
\begin{align}
{\tilde F_K}\le\sum_{h\neq k}\rho_h^Ku_h+\rho_k^KR.
\label{eq_Ftilde<uk}
\end{align}
Second, a (possibly empty) subset of the following constraints, which $(u,v)$ satisfies, are removed:
\begin{subequations}
\begin{align}
&{\tilde F_K}\le\sum_{h\neq \ell}\rho_h^Ku_h+\rho_\ell^KR,
\quad\mbox{if }
\ell<k
\mbox{ and }
\sum_{h=1}^\ell\rho_h^Ku_h+\sum_{h=\ell+1}^K\rho_h^Ku_hv_h>F-\Delta,
\label{eq_Ftilde<u}\\
&{\tilde F_K}\le\sum_{h=\ell+1}^K\rho_h^Ku_h+\rho_\ell^KF,\quad\mbox{if }
\ell<k
\mbox{ and }
\sum_{h=1}^\ell\rho_h^Ku_h+\sum_{h=\ell+1}^K\rho_h^Ku_hv_h>F-\Delta,
\label{eq_Ftilde<Fk}
\end{align}
\end{subequations}
One can obtain from \eqref{eq_minF-x<} that \eqref{eq_Ftilde<u}--\eqref{eq_Ftilde<Fk} implies \eqref{eq_Ftilde<uk}. Therefore, if $(u,v)$ satisfies \eqref{eq_stable1a}--\eqref{eq_stable1z}, so does $(u,v')$.
$\quad\blacksquare$

%Now we show a condition under which the sufficient condition is also necessary.
%Suppose that the demand vector $d$ satisfies the following condition:
%\begin{cnd}
%\label{cnd_1bn}
%For each $k$, either
%\begin{align}
%F-u\le\sum_{h=1}^{k}\rho_h^k d_h\le\frac{(F-\Delta)}{\rho_{k}^K}
%\label{eq_pm}
%\end{align}
%or
%\begin{align}
%(1-\rho_{k-1})F\le d_k\le \frac{(F-\Delta)}{\rho_k^K}
%\label{eq_po}
%\end{align}
%holds.
%\end{cnd}
%The inequality \eqref{eq_pm} (resp. \eqref{eq_po}) essentially ensures that the $k$-th on-ramp (resp. the $(k-1)$-th mainline cell) is not a potential bottleneck.
%If they are simultaneously potential bottlenecks, the highway necessarily has realized bottlenecks.
%Then, we have the following result:
%\begin{cor}
%\label{cor_1}
%Consider a highway with a stationary hotspot and a control scheme $(x,v_x^*)$ satisfying Condition \ref{cnd_1bn}.
%Then, the highway is stable if and only if
%\begin{align}
%%\sum_{h=1}^k\rho_h^kd_h<F,\;k=2,3,\ldots,n-1,\;
%\sum_{h=1}^K\rho_h^Ku_h<\sfp_1F+\sfp_2 (F-\Delta).
%\label{eq_drift1}
%\end{align}
%\end{cor}
%
%\begin{pf}
%\noindent\emph{Sufficiency:}
%
%Lemma~\ref{lmm_Scal2} in the appendix gives an invariant set $\Scal_1$ for highways satisfying Condition~\ref{cnd_1bn}.
%For each $(q,{n})\in\Scal$ such that $q\neq0$, by Lemma~\ref{lmm_Scal2}, we have
%\begin{align*}
%f_K(1,q,n)=F.
%\end{align*}
%for every ${\tilde F_K}$ satisfying \eqref{eq_stable2} and \eqref{eq_stable3}.
%Then, consider the Lyapunov function
%\begin{align}
%V&=(q+{n})^T
%\left[\begin{array}{ccccc}
%\rho_1^K & \rho_2^K & \rho_3^K & \cdots & \rho_K^K\\
%\rho_2^K & \rho_3^K & \rho_4^K & \cdots & 1/\rho_1^2\\
%\rho_3^K & \rho_4^K & \rho_5^K & \cdots & 1/\rho_1^3\\
%\vdots & \vdots & \vdots & \ddots & \vdots\\
%\rho_{n-1}^K & \rho_K^K & 1/\rho_1^2 & \cdots & 1/\rho_1^{n-1}\\
%\rho_K^K & 1/\rho_1^2 & 1/\rho_1^2 & \cdots & 1/\rho_1^K
%\end{array}\right]
%(q+{n})\nonumber\\
%&\quad-(-1)^i(\sfp_1F-\sfp_2(F-\Delta))\left[\begin{array}{ccccc}\rho_K^K & 1/\rho_1^2 & 1/\rho_1^2 & \cdots & 1/\rho_1^K
%\end{array}\right](q+{n});
%\label{eq_V2}
%\end{align}
%note that the only difference from the Lyapunov function defined in \eqref{eq_V1} is that ${\tilde F_K}$ is replaced by $F$. The rest of the proof is analogous to that of Theorem~\ref{thm_stable1}.
%
%\noindent\emph{Necessity:}
%
%The necessity of $\sum_{k=1}^K\rho_k^Kd_k\le(\sfp_1 F+\sfp_2(F-\Delta))$ is obvious; otherwise $\lim_{t\to\infty}|q(t)|=\infty$ a.s. To exclude the equality, suppose that $\sum_{k=1}^K\rho_k^Kd_k=(\sfp_1 F+\sfp_2(F-\Delta))$. Then, for each initial condition $Q(0)=q$ and $N(0)=n$, we have
%\begin{align*}
%\sum_{k=1}^K\rho_k^Kq_k(t)&=\sum_{k=1}^K\rho_k^Kq_k+\int_{{s}=0}^t\left(\sum_{k=1}^K\rho_k^Kd_k-f_K({s})\right)d{s}\\
%&\ge\sum_{k=1}^K\rho_k^Kq_k+\int_{{s}=0}^t\left(\sum_{k=1}^K\rho_k^Kd_k-F({s})\right)d{s}\\
%&=\sum_{k=1}^K\rho_k^Kq_k+\left(\sum_{k=1}^K\rho_k^Kd_k-(\sfp_1 F+\sfp_2(F-\Delta))\right)t\quad a.s.\\
%&=\sum_{k=1}^K\rho_k^Kq_k.
%\end{align*}
%Hence, we have
%\begin{align*}
%\limsup_{t\to\infty}\frac1t\int_{{s}=0}^t\E[|Q({s})|]d{s}
%\ge\limsup_{t\to\infty}\frac1t\int_{{s}=0}^t\E\left[\sum_{k=1}^K\rho_k^KQ_k({s})\right]d{s}
%\ge\sum_{k=1}^K\rho_k^Kq_k.
%\end{align*}
%Thus, for any positive constant $C$, there exists an initial condition $Q_K(0)=2C$ such that
%\begin{align*}
%\limsup_{t\to\infty}\frac1t\int_{{s}=0}^t\E[|Q({s})|]d{s}
%>C,
%\end{align*}
%which implies that the highway is not stable.
%
%\end{pf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{exm}[I210-EB, stationary]

This example illustrates Theorem~\ref{thm_stable1} and Propositions~\ref{prp_nec1} and \ref{prp_ystar1}, and visualizes the structure of the throughput-maximizing problem \eqref{eq_thpmax1}.
%figure
\begin{figure}[hbt]
\centering
\subfigure[The S. Mountain Ave. on-ramp to I210.]{
\centering
\includegraphics[width=0.35\textwidth]{./Images/fig_exm2}
\label{fig_exm2}
}
\subfigure[The model for the on-ramp.]{
\centering
\includegraphics[width=0.35\textwidth]{./Images/fig_exm2_CTM}
\label{fig_exm2_CTM}
}
%\subfigure[The mode transitions.]{
%\centering
%\includegraphics[width=0.2\textwidth]{./Images/fig_chain}
%\label{fig_chain}
%}
\caption{Traffic control for a stationary hotspot on I210.}
\label{fig_exm2}
\end{figure}
Consider the South Mountain Avenue on-ramp to I210 East-bound in Monrovia, California, USA as shown in Figure~\ref{fig_exm2}. Calibrated model parameters are available in Table~\ref{tab_parameters1}.
\begin{table}[hbt]
\centering
\caption{Parameters of the CTM shown Figure~\ref{fig_exm2_CTM}.}
\label{tab_parameters1}
\begin{tabular}{@{}lllll@{}}
\toprule
Quantity & Free-flow speed $\alpha$ & Nominal capacity $F$, $R$ & Capacity reduction $\Delta$ &Jam density $n^\max$ \\ \midrule
Cell 1    & 108 km/hr       & 7360 veh/hr    & N/A & 354 veh/km  \\ 
Cell 2    & 111 km/hr       & 9850 veh/hr   & 1970 veh/hr & 411 veh/km  \\ 
Buffer 1    & N/A       & 7360 veh/hr    & N/A & N/A  \\ 
Buffer 2    & N/A       & 3000 veh/hr    & N/A & N/A \\
\bottomrule
\end{tabular}
\end{table}
We use this example to illustrate how the control scheme $(u,v)$ affects the stability of the on-ramp/upstream queues, and provides insights for the max-throughput problem~\eqref{eq_thpmax1}.

\begin{figure}[htb]%Two-cell segment
\centering
\includegraphics[width=0.45\textwidth]{./Images/fig_stable1}
\caption{Stability of various control schemes $(u,v)$. The boundary between regions 1 and 2 is the margin criterion for ramp control given by Proposition~\ref{prp_ystar1}.}
\label{fig_stable1}
\end{figure}

\begin{table}[hbt]
\centering
\caption{Stability of various regions in Figure~\ref{fig_stable1}.}
\label{tab_stable1}
\begin{tabular}{@{}llll@{}}
\toprule
Region & Mainline priority ($v_2=0)$ & Baseline ($v_2=1$) & Margin criterion ($v_2={y}^*_2)$ \\ \midrule
1 \& 2      & Stable                     & Stable                                  & Stable                 \\
3      & Unknown                     & Stable                                  & Stable                 \\
4      &   Stable                   & Unknown                                 & Stable                 \\
5      &    Unstable                 &     Unstable                              & Unstable                               \\ \bottomrule
\end{tabular}
\end{table}

For each $(u,v)$, we can verify the stability by applying Proposition~\ref{prp_nec1} and Theorem~\ref{thm_stable1}.
Fig.~\ref{fig_stable1} shows the results; the meaning of each region is listed in Table~\ref{tab_stable1}.
Specifically, if a given $(u,v)$ verifies the sufficient condition Theorem~\ref{thm_stable1}, then it is labeled as ``stable''; if it does not verify the necessary condition Proposition~\ref{prp_nec1}, then it is labeled as ``unstable''; if it verifies the necessary condition but not the sufficient condition, then it is labeled as ``unknown''.
This figure also shows the margin criterion, which is the boundary between regions 1 and 2: $v_2^*=0$ in regions 2 and 4, and $v_2^*=1$ in regions 1 and 3.

Figure~\ref{fig_stable1} in fact visualizes the feasible set to the problem~\eqref{eq_thpmax1}. For example, if $v_2=1$, then the feasible set for $x$ is regions 1--3. For each given demand vector $d=[d_1,d_2]^T$, one can also graphically determine the optimal control scheme. For example, if $d$ lies in region 1, then $(u,v)\in\{d\}\times\{0,1\}^2$ are all optimal solutions; if $d$ lies in region 3, then $u=d$, $v=[1,1]^T$ is an optimal solution; if $d$ lies in region 5, then not all demand can be accepted, but one can draw a set of ``iso-throughput'' curves to determine the optimal solution.

We note two important facts here.
First, the margin criterion for ramp metering, i.e. ${y}^*$, is an optimal solution to the max-throughput problem~\eqref{eq_thpmax1}, regardless of the demand vector $d$.
Second, under $y^*$, there is no gap between the stable regions (1--4) and the unstable region 5, and the sufficient condition is also necessary. Hence, ${y}^*$ attains the actual maximal throughput.
The former fact is true for all highways with a single perturbation hotspot, but the latter is in general not true; there may be a gap between the necessary condition and the sufficient condition if the model parameters are varied.

\end{exm}

%----------------------------------------------
\subsection{Moving bottlenecks}

For moving bottlenecks, tractable analysis for a general $K$-cell highway is not easy, since the number of modes and the dimension of $q$ and $n$ increase with $K$.
Instead, we consider a single merge, i.e. a two-cell highway section with an upstream buffer and an on-ramp buffer.
Then, we obtain the ``margin criterion'' for traffic control under moving bottlenecks:

\begin{prp}[Margin criterion, moving]
\label{prp_ystar2}
Consider a single merge with moving bottlenecks. Suppose that $(u^*,v^*)$ is an optimal solution.
\begin{enumerate}
\item The ramp control scheme $v^\dagger=[1,1]^T$ is also optimal if
\begin{align}
R-u_2^*\le \rho_{1}(F-\Delta-u_1^*).
\label{eq_moving_margin1}
\end{align}
\item The ramp control scheme $v^\dagger=[1,0]^T$ is also optimal if
\begin{align}
R-u_2^*\ge \rho_{1}(F-u_1^*).
\label{eq_moving_margin2}
\end{align}
\end{enumerate}
\end{prp}

The above result essentially states that, if the on-ramp has a capacity-demand margin ($R-u_2^*$) smaller than the mainline even under the influence of the moving bottleneck $\rho_1(F-\Delta-u_1^*)$, then it is supposed to be metered; if the on-ramp has a capacity-demand margin ($R-u_2^*$) larger than the mainline even without the influence of the moving bottleneck $\rho_1(F-u_1^*)$, then it is not supposed to be metered.
If the margins do not fall in the above regimes, this result does not provide conclusive characterization of the structure of the optimal ramp metering plan.

The above result essentially states that, if the $k$th on-ramp has a capacity-demand margin ($R-u_k^*$) smaller than the mainline even under the influence of the moving bottleneck $\rho_{k-1}(\underline F_{k-1}-\sum_{h=1}^k\rho_h^ku_h^*)$, then it is supposed to be metered; if the on-ramp has a capacity-demand margin ($R-u_k^*$) larger than the mainline even without the influence of the moving bottleneck $\rho_{k-1}(\overline F_{k-1}-\sum_{h=1}^k\rho_h^ku_h^*)$, then it is not supposed to be metered.
If the margins do not fall in the above regimes, this result does not provide conclusive characterization of the structure of the optimal ramp metering plan.
However, we can still obtain the optimal solution by implementing algorithms for solving the MILP \eqref{eq_thpmax2}.

\noindent{\bf Proof of Proposition~\ref{prp_ystar2}}
This proof is based on the stability conditions given by Theorem~\ref{thm_stable2}.
This proof is based on the stability conditions given by Theorem~\ref{thm_stable2}.

\noindent{Part (1).}
If $v^*=[1,1]^T$, then $v^\dagger$ is indeed optimal. Suppose that $v^*=[1,0]^T$, and that there exist $a^*_k,b^*_i,\tilde f_k^*(i,{x},{y})$, and $\tilde r_k^*(i,{x},{y})$ that verify \eqref{eq_stable2a}--\eqref{eq_stable2z}.
Then, the following inequalities hold:
\begin{subequations}
\begin{align}
& \tilde f_1^*(i,[0,1]^T,[0,0]^T)\le u_1^*,\label{eq_fstar1}\\
& \tilde f_2^*(i,[0,1]^T,[\cdot,0]^T)\le\rho_1u_1^*+R.\label{eq_fstar2}
\end{align}
\label{eq_fstar}%
\end{subequations}

If we change $v_2$ from 0 to 1, then \eqref{eq_fstar1} and \eqref{eq_fstar2} (more precisely, their counterparts for $f^\dagger$) are no longer involved (because of \eqref{eq_theta}).
Instead, the following inequalities have to hold:
\begin{subequations}
\begin{align}
& \tilde f_1(i,[1,0]^T,[\cdot,0]^T)\le F,\label{eq_fdagger1}\\
& \tilde f_2(i,[1,0]^T,[\cdot,0]^T)\le\rho_1(F-\Delta)+u_2.\label{eq_fdagger2}
\end{align}
\label{eq_fdagger}%
\end{subequations}
The other inequalities imposed on $f^*$ are not affected.

Let
\begin{align}
&f_k^\dagger(i,{x},{y})=\left\{\begin{array}{ll}
\tilde f_k^*(i,[0,1]^T,{y}), & {x}=[1,0]^T,{y}_2=0,\\
\tilde f_k^*(i,{x},{y}), & \mbox{o.w.}
\end{array}\right.
\end{align}
Then, one can obtain from \eqref{eq_moving_margin1} and \eqref{eq_fstar} that $f^\dagger$ as defined above satisfies \eqref{eq_fdagger1} and \eqref{eq_fdagger2}.
Hence, given the decision variables $(u^*,v^\dagger)$, and together with the constants $\alpha^*_k,\gamma^*_i,\tilde r_k^*(i,{x},{y})$, the constants $f_k^\dagger(i,{x},{y})$ also verify the stability conditions in Theorem~\ref{thm_stable2}.
That is, $(u^*,v^\dagger)$ is also a feasible solution to the problem \eqref{eq_thpmax2}. Since $x^*$ maximizes the throughput $J$, $(u^*,v^\dagger)$ is an optimal solution.

\noindent{Part (2).} The proof is analogous to that of Part (1).
$\quad\blacksquare$

\begin{exm}[Moving bottlenecks on I210-EB]
This example illustrates Theorem~\ref{thm_stable2} and Propositions~\ref{prp_nec2} and \ref{prp_ystar2}, and visualizes the structure of the throughput-maximizing problem \eqref{eq_thpmax2}.
%%figure
%\begin{figure}[hbt]
%\centering
%\subfigure[The S. Mountain Ave. on-ramp to I210.]{
%\centering
%\includegraphics[width=0.35\textwidth]{./Images/fig_exm2}
%\label{fig_exm2}
%}
%\subfigure[The model for the on-ramp.]{
%\centering
%\includegraphics[width=0.35\textwidth]{./Images/fig_exm2_CTM}
%\label{fig_exm2_CTM}
%}
%%\subfigure[The mode transitions.]{
%%\centering
%%\includegraphics[width=0.2\textwidth]{./Images/fig_chain}
%%\label{fig_chain}
%%}
%\caption{Traffic control for a stationary hotspot on I210.}
%\label{fig_merge}
%\end{figure}
Consider again the South Mountain Avenue on-ramp to I210 East-bound in Monrovia, California, USA, as illustrated in Figure~\ref{fig_merge}.
We use this example to illustrate how the control scheme $(u,v)$ affects the stability of the on-ramp/upstream queues, and provides insights for the max-throughput problem~\eqref{eq_thpmax2}.

For each $(u,v)$, we can verify the stability by applying Proposition~\ref{prp_nec1} and Theorem~\ref{thm_stable1}.
Figure~\ref{fig_stable1} shows the results; the meaning of each region is listed in Table~\ref{tab_stable1}.
Specifically, if a given $(u,v)$ verifies the sufficient condition Theorem~\ref{thm_stable1}, then it is labeled as ``stable''; if it does not verify the necessary condition Proposition~\ref{prp_nec1}, then it is labeled as ``unstable''; if it verifies the necessary condition but not the sufficient condition, then it is labeled as ``unknown''.
This figure also shows the margin criterion, which is the boundary between regions 1 and 2: $v_2^*=0$ in regions 2 and 4, and $v_2^*=1$ in regions 1 and 3.

%\begin{figure}[htb]%Two-cell segment
%\centering
%\includegraphics[width=0.45\textwidth]{./Images/fig_stable}
%\caption{Stability of various demand patterns under various ramp control strategies.}
%\label{fig_stable2}
%\end{figure}

\begin{figure}[hbt]
\subfigure[Mainline priority.]{
\centering
\includegraphics[width=0.3\textwidth]{./Images/fig_stable}
\label{vht_baseline}
}
\subfigure[ALINEA v.s. baseline.]{
\centering
\includegraphics[width=0.3\textwidth]{./Images/thp_op}
\label{thp_op}
}
\subfigure[Mainline priority v.s. baseline.]{
\centering
\includegraphics[width=0.3\textwidth]{./Images/vht_op}
\label{vht_op}
}
\caption{Throughput induced by mainline priority/ALINEA compared to baseline. Red (resp. blue) means lower (resp. higher) throughput than baseline.}
\label{fig_exm}
\end{figure}

\begin{table}[hbt]
\centering
\caption{Stability of various regions in Figure~\ref{fig_stable2}.}
\label{tab_stable2}
\begin{tabular}{@{}llll@{}}
\toprule
Region & Ramp metered $v_2=0$ & Ramp not metered $v_2=0$ & Margin criterion $v_2^*$ \\ \midrule
1      & Stable                     & Stable                                  & Stable                 \\
2      & Unknown                     & Stable                                  & Stable/unknown                 \\
3      &   Stable                   & Unknwon                                 & Stable                 \\
4      &   Unknown                   & Unknown                                 & Unknown                \\
5      &    Unstable                 &     Unstable                              & Unstable                               \\ \bottomrule
\end{tabular}
\end{table}

Figure~\ref{fig_stable1} in fact visualizes the feasible set to the problem~\eqref{eq_thpmax1}. For example, if $v_2=1$, then the feasible set for $x$ is regions 1--3. For each given demand vector $d=[d_1,d_2]^T$, one can also graphically determine the optimal control scheme. For example, if $d$ lies in region 1, then $(u,v)\in\{d\}\times\{0,1\}^2$ are all optimal solutions; if $d$ lies in region 3, then $x=d$, $y=[1,1]^T$ is an optimal solution; if $d$ lies in region 5, then not all demand can be accepted, but one can draw a set of ``iso-throughput'' curves to determine the optimal solution.

We also simulated the throughput and VHT resulting from the margin criterion. In the simulation, mainline is prioritized only if \eqref{eq_moving_margin2} holds. 
Comparison between Figures~\ref{thp_op} and \ref{thp_bl}--\ref{thp_mp} implies that the margin criterion maintains the VMT.
Comparison between Figures~\ref{vht_op} and \ref{vht_bl}--\ref{vht_mp} implies that the margin criterion significantly reduces travel delay and essentially maintain bounded queues at the on-ramp and at the upstream entrance.

%We note two important facts here.
%First, the margin criterion for ramp metering, i.e. ${y}^*$, is an optimal solution to the max-throughput problem~\eqref{eq_thpmax1}, regardless of the demand vector $d$.
%Second, under $y^*$, there is no gap between the stable regions (1--4) and the unstable region 5, and the sufficient condition is also necessary. Hence, ${y}^*$ probably attains the actual maximal throughput.
%The former fact is true for all highways with a single perturbation hotspot, but the latter is in general not true; there may be a gap between the necessary condition and the sufficient condition if the model parameters are varied.

%The result illustrates the essence of the ramp control policy $\mu^*$. One can see from Figure~\ref{fig_stable2}: (i) when $D_1$ is relatively large, the mainline should be prioritized (Region 5); (ii) when $D_2$ is relatively large, the on-ramps should be prioritized (Regions 3 and 4).
%The criterion involved in $\mu^*$ essentially approximates the boundary between the above two cases with a simple inequality.
%Recall from Theorem~\ref{thm_single2} that this approximation is exact for single-hotspot highways.
%For multi-hotspot highways such as the one considered here, this approximation slightly deviates from the actual boundary.

%Finally, one can compare Figures~\ref{} and Figure~\ref{fig_stable2} to further interpret the above-mentioned rationale of the margin criterion.
\end{exm}
